Neural Font Rendering

Recent advances in deep learning techniques and applications have revolutionized artistic creation and manipulation in many domains (text, images, music); however, fonts have not yet been integrated with deep learning architectures in a manner that supports their multi-scale nature. In this work we aim to bridge this gap, proposing a network architecture capable of rasterizing glyphs in multiple sizes, potentially paving the way for easy and accessible creation and manipulation of fonts.

==> figures/resizing-comparison-upscaled.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/resize_issues}
  \caption{\ohad{The (a), (b), ... labels in the image are too small.} Upscaled comparison of several image resizing techniques applied to rendered glyphs.
  (a) Tahoma glyph 'm' rendered in pointsize 16.
  (b) - (f) Tahoma glyph 'm' rendered in pointsize 24 and resized to same size of (a) with the following techniques, respectively: (b) nearest neighbor, (c) bilinear interpolation, (d) Hamming interpolation, (e) bicubic interpolation, (f) Lanczos resampling. }
  \label{resize-issues}
\end{figure}

==> figures/resizing-comparison.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/resize_issues_small}
  \caption{\ohad{The Q looks weird because it's above the baseline.} \ohad{It's extremely hard to see the differences. I would pick a few letters and show them, much larger, and perhaps with diff images or zoomed-in regions. The next figure has that for one letter, but I think that's going too far to the other extreme. Instead of the two figures, use only one figure with a few letters in it. Pick the number of letters such that the artifacts are still visible, but try to fit more than a couple of glyphs. The two figures you currently have can move to supplementals.} Comparison of several image resizing techniques applied to rendered glyphs.
  (a) Tahoma glyphs rendered in pointsize 16.
  (b) - (f) Tahoma glyphs rendered in pointsize 24 and resized to same size of (a) with the following techniques, respectively: (b) nearest neighbor, (c) bilinear interpolation, (d) Hamming interpolation, (e) bicubic interpolation, (f) Lanczos resampling. }
  \label{resize-issues-small}
\end{figure}


==> figures/vector-glyph-rasterization-upscaled.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/hinting_importance}
  \caption{Upscaled comparison of vector glyph rasterization (a) with hinting and (b) without hinting. The glyph is Times New Roman 'm', pointsize 14. The differences are prominent, e.g. note the top of the glyphs, where in the unhinted version the arches are blurred and unclear, as opposed to the hinted version.}
  \label{hinting-importance}
\end{figure}


==> figures/vector-glyph-rasterization.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/hinting_importance_small}
  \caption{\ohad{Same comment as for the 2 previous figures. No need to use two figures to show this phenomena. Create one figure, with a reasonable number of glyphs.} Comparison of vector glyph rasterization (a) with hinting and (b) without hinting. The face is Times New Roman, pointsize 14. Inconsistencies in style are observable, e.g. the serifs of 'U' and 'V' are hardly visible, among other issues. }
  \label{hinting-importance-small}
\end{figure}

==> font-rendering-original.tex <==



\section{Background on Font Rendering}
\label{sec:font-rendering}

Fonts constitute a fundamental cornerstone in today's highly digital world, with tens of thousands of font families being available, expressing a great diversity in design, style, and typical use. Most fonts support hundreds to thousands of glyphs, including multiple alphabets, accented versions of letters, punctuation marks, and other symbols. Fonts are also often displayed in multiple sizes.

As a result, the most naïve font representation scheme, as a collection of images of all supported glyphs in all supported sizes, is highly infeasible, both in terms of storage space and the resultant amount of work for typeface designers.

A feasible alternative would be to persist glyph images in only several key sizes, and use image resizing techniques to interpolate to other sizes. However, such a method introduces undesired artifacts, compromising glyph quality (\Cref{resize-issues-small,resize-issues}).

\input{figures/resizing-comparison}

\input{figures/resizing-comparison-upscaled}

These issues are resolved by representing glyph outlines as vector graphics, i.e. sets of mathematical curves; such a representation is trivial to scale. Unfortunately, vector representation alone is not sufficient for high-quality glyph rendering, especially for small font sizes, as the rasterization process can also introduce artifacts (\Cref{hinting-importance-small,hinting-importance}). To address that, modern font formats support \textit{hints} --- systems of instructions defined by the typeface designer, which are used to modify the glyph outline after scaling but prior to rasterization, in order to better align it with the rasterized grid and avoid undesired artifacts.

\input{figures/vector-glyph-rasterization}

\input{figures/vector-glyph-rasterization-upscaled}

In the next two subsections, we will further explain the vector representation of glyphs and give an overview of hinting techniques, respectively.
\subsection{Vector Glyph Outlines}
Modern digital display screens are mostly based on raster graphics, displaying matrix representations of images via rectangular arrays of pixels. Therefore, the most straightforward approach to representing the glyphs of a certain font would involve persisting the glyphs' matrix representations. As previously discussed, this approach leads to very large and impractical font sizes due to resizing artifacts and the need to render fonts in multiple scales.

The resizing and pixelation issues are not unique to font rendering, and are generally solved by representing images in an alternative format, based on \textit{vector graphics}. Such formats represent shapes as mathematical objects --- lines, circles, curves, etc. in some canonical scale. When an image represented by vector graphics is to be rendered, the mathematical representation is first scaled based on the rendering dimensions, and then drawn to a matrix representation via a process called \textit{rasterization}.

Most type formats represent glyphs by the vector graphics representation of their outlines. Specifically, the outline contours are typically represented by collections of lines and Bézier curves. Conveniently, such a representation can be achieved by persisting ordered collections of points, along with tags indicating which points are part of the contour and which points are Bézier control points.

\input{figures/glyph-outlines}

\Cref{vector-representation} depicts the outlines of three glyphs, along with the points used to describe their outlines. Blue points denote points that exactly lie on the outline, while red points denote curve control points.

\subsection{Hinting}
As previously discussed and demonstrated, vector representation of glyph outlines is not sufficient to achieve precise rasterization of glyphs, especially in small sizes or resolutions. The hinting process aims at resolving these issues by applying modifications to the glyph outlines, after scaling but prior to rasterization. These modifications primarily better align the outline to the rasterized pixel grid. \Cref{hinting-outline} demonstrates the effects of hinting on several glyph outlines.

Glyph hints are created as part of the type design process, either using automatic hinting techniques available in the editor, or by the typeface designer.
The types of hints, and the ways they are applied, differ between type formats. Typically, hinting systems provide a set of instructions which are applied to the outline after scaling. These instructions are used to specify constraints or rules for various points defining the outline; for example, justification of a point based on the global glyph height, or specifying a minimum distance between two points.

Overall, the resulting glyph rendering process is quite involved, generally consisting of the following steps:
\begin{itemize}
    \item Scaling the vector representation of the glyph outline
    \item Applying hints to the glyph outline
    \item Rasterizing the outline onto the pixel grid
\end{itemize}


We propose an approach for simplifying the glyph rendering process while satisfying all the requirements that led to the complexity of current approaches.

==> intro.tex <==
\section{Introduction}
Typefaces have become ubiquitous --- you can choose from hundreds of different digital-font alternatives to suit your style and need. After choosing a font, you can pick any size of characters you want and the glyph images appear on your screen. Behind the scenes, fonts are not represented using bitmaps of various sizes. Instead, the glyphs are defined using vector-based curves that represent the outline of their boundary. To create bitmaps in a given size, a complex procedure called character rasterization is applied, converting the continuous representation of the glyphs to bitmaps (\Cref{fig:rasterization}). First, scaling is performed by overlaying a suitable-size grid of pixels on the outline of the glyph, and then appropriate pixels are chosen to represent the shape of the glyph. However, simply turning on the pixels that are inside the outline creates noticeable artifacts that lower the glyph quality and legibility (e.g., \Cref{hinting-importance}). Therefore, before converting to pixels, the outline of the glyph is modified to better align with the rasterization grid, and only then the pixels are sampled. This process is called grid-fitting and it is governed by what is often called \textit{hints} --- commands that modify the outline's shape to better fit the grid of pixels and preserve typographic constraints such as maintaining widths and distances of glyph elements. Thus, each glyph within a digital font is not defined by a vector outline only, but includes complex hints that support fitting it to all sizes, written in a specialized programming language such as TrueType or PostScript. 

All this means that the process of rasterization of glyphs is intricate and cannot be defined by simple rules.  
Such complex functions are where neural networks were found to work well. 
In this work, we investigate the possibility of representing fonts using a deep neural network capable of rendering high quality glyphs \emph{in all sizes}. Although previous works already presented neural networks for various font manipulations (e.g., \cite{Bernhardsson2016,Jiang2019SCFontSC,Park2018TypefaceCW,Upchurch16,Xi20} and more), these works focus on a specific point size and manipulate glyph renderings in that size in the image domain. We wish to present a multi-scale representation of fonts that can be used in any size, similar to current digital fonts. 

Given a glyph id in some font, we can define our goal as representing a function $f$ that, given a size will produce the image of the glyph (i.e., the ``bitmap'') in that size: 
$$
I^{size} = f(id,size) = f_{id}(size) 
$$
Using such a representation, the whole image is synthesized as the output of $f$.

Alternatively, we can formulate the problem using an implicit representation of a specific glyph, where the rendering process involves sampling the implicit representation at multiple positions. Recently, implicit models have gained popularity in computer vision. In such a representation, the object is modeled as an implicit function $g$ that can be sampled in space. A glyph can be represented in a similar manner, only the size of the sampling grid must also be given as input:
$$
I^{size}[i,j] = g_{id}(i,j,size) 
$$
Such representation allows the creation of the glyph bitmap by sampling all the pixels for a given size in a specified bounding box. 

In this work, we explore both formulations (direct and implicit).


One of the major difficulties in representing glyphs is that in order for them to be legible, the quality of the resulting bitmaps must be perfect in all sizes. Due to the nature of glyphs (small, monochromatic, with clear edges), even small errors are noticeable, and we cannot have glyphs that look good only in some sizes.
This constraint imposes strong restrictions on the error rate of the network, and makes font synthesis fundamentally different from natural image synthesis. 


These are our primary considerations in this work:
\begin{itemize}
    \item Near-zero error rate: to be practically useful as a font rasterization tool, the model error (pixelwise difference between the ground truth glyph and the reconstructed glyph) must be extremely small, to a degree that is unnoticeable for all readers. This is different from many machine learning settings, where a certain error tolerance exists.
    \item Multi-scale output: The model architecture needs to support rasterizing glyphs in a wide range of sizes. While it is possible to always generate images of the largest possible size, padded appropriately (to account for the desired size), this isn't necessarily the optimal approach; in this work, we explore this option, and also an approach that utilizes an implicit glyph representation and sampling to implement the multi-scale rasterization requirement.
    \item Generalization: While we are interested in near-zero error for reconstructed glyphs, we are also interested in using the model to interpolate between fonts and font weights, and as such need to be able to represent a rich font space, and train the model in a manner that will allow it to generalize when sampled out-of-training-distribution. To achieve that we utilize elements from generative adversarial network (GAN) \cite{goodfellow2014generative} training.
\end{itemize}

If successful, we would show that networks are inherently capable of representing the adaptations necessary to render high-quality glyphs in a wide range of sizes. This in turn could pave the way to hint-free font design and usage, which could greatly simplify the typeface design process.

\input{figures/rasterizing-glyphs}

